Only Encode Once: Making Content-based News Recommender Greener

Large pretrained language models (PLM) have become de facto news encoders in modern news recommender systems, due to their strong ability in comprehending textual content. These huge Transformer-based architectures, when finetuned on recommendation tasks, can greatly improve news recommendation performance. However, the PLM-based pretrain-finetune framework incurs high computational cost and energy consumption, primarily due to the extensive redundant processing of news encoding during each training epoch. In this paper, we propose the ``Only Encode Once'' framework for news recommendation (OLEO), by decoupling news representation learning from downstream recommendation task learning. The decoupled design makes content-based news recommender as green and efficient as id-based ones, leading to great reduction in computational cost and training resources. Extensive experiments show that our OLEO framework can reduce carbon emissions by up to 13 times compared with the state-of-the-art pretrain-finetune framework and maintain a competitive or even superior performance level. The source code is released for reproducibility.

==> plots/param/appearance-v2.tex <==

\begin{tikzpicture}

    \begin{groupplot}[
        group style={
            group name=my fancy plots,
            group size=1 by 2,
            xticklabels at=edge bottom,
            vertical sep=0pt
        },
        width=8.5cm,
        % line width=0.35mm,
        xtick={0, 2000, 4000, 6000},
        xticklabels={0, 2, 4, 6},
        xmin=0,
        xmax=7000,
        xlabel=Carbon Emission (Kg),
        ylabel=AUC,
        xmajorgrids=true,
        ymajorgrids=true,
        grid style=dashed,
        legend columns=2,
        legend style={
            font=\normalsize,
            legend cell align=left,
        },
        legend pos=south east,
    ]
    
    \nextgroupplot[
        ymin=63,
        ymax=66,
        ytick={64, 66},
        axis x line=top, 
        axis y discontinuity=parallel,
        height=6.0cm,
        xlabel=,
        y label style={at={(-0.1,0.1)}},
    ]
        % NRMS
        \addplot[color=fuguang, only marks, style={mark=*, fill=fuguang,mark size=4pt}] coordinates {(1010,64.12)};\label{plot:nrms}
        % \addlegendentry{}
        % DCN
        \addplot[color=fuguang, only marks, style={mark=triangle*, fill=fuguang,mark size=5pt}] coordinates {(1684,63.88)};\label{plot:dcn}
        % \addlegendentry{$\texttt{Text-based}$}
        
        % NRMS-PLMNR
        \addplot[color=qingdai, only marks, style={mark=*, 
        fill=qingdai,mark size=4pt}] coordinates {(4043,65.57)};\label{plot:nrms-plm}
        % \addlegendentry{}
        % DCN-PLMNR
        \addplot[color=qingdai, only marks, style={mark=triangle*, fill=qingdai,mark size=5pt}] coordinates {(6570,65.42)};\label{plot:dcn-plm}
        % \addlegendentry{$\texttt{PLM-plugged}$}
        
        % NRMS-MFT
        \addplot[color=zhucao, only marks, style={mark=*, fill=zhucao,mark size=4pt}] coordinates {(505,64.34)};\label{plot:nrms-gnrs}
        % \addlegendentry{}
        % DCN-MFT
        \addplot[color=zhucao, only marks, style={mark=triangle*, fill=zhucao,mark size=5pt}] coordinates {(1010,65.44)};\label{plot:dcn-gnrs}
        % \addlegendentry{$\texttt{GNR-based}$}      
    
    \nextgroupplot[
        ymin=56,ymax=58,
        ytick={56, 58},
        axis x line=bottom,
        height=4.0cm,
        ylabel=,
    ]
        % NRMS-id
        \addplot[color=tushoulan, only marks, style={mark=*, fill=tushoulan,mark size=4pt}] coordinates {(471,57.59)}; \label{plot:nrms-id}
        % \addlegendentry{}
        % DCN-id
        \addplot[color=tushoulan, only marks, style={mark=triangle*, fill=tushoulan,mark size=5pt}] coordinates {(791,57.41)};\label{plot:dcn-id}
        % \addlegendentry{$\texttt{ID-based}$}
    \end{groupplot}
    
        \node[draw,fill=white,inner sep=4pt,above left=0.5em] at (6.7, -2.4) {
        \setlength\tabcolsep{2pt}
        \begin{tabular}{ccl}
        $\texttt{NRMS}$ & $\texttt{DCN}$ \\
        \ref{plot:nrms-id} & \ref{plot:dcn-id} & $\texttt{ID-based}$\\
        \ref{plot:nrms} & \ref{plot:dcn} & $\texttt{Text-based}$\\
        \ref{plot:nrms-plm} & \ref{plot:dcn-plm} & $\texttt{PLM-based}$ \\
        \ref{plot:nrms-gnrs} & \ref{plot:dcn-gnrs} & $\texttt{GNR \small{(ours)}}$
        \end{tabular}
        };
\end{tikzpicture}


==> plots/percentage/main.tex <==
% \definecolor{lightc}{rgb}{0.86, 0.90, 0.94}

% % \begin{figure}[t]
% % \centering
% % \setlength\tabcolsep{0pt}

% % \resizebox{0.6\linewidth}{!}{
% % \begin{tabular}{c}

% \begin{tikzpicture}
%     \begin{axis}[
%         ylabel=News Articles \%,
%         xlabel=$\#Appearance$,
%         line width=0.35mm,
%         grid=both,
%         grid style=dashed,
%     ]

%         \draw[
%             purple!80!white,
%             dashed,
%             line width=0.6mm,
%             opacity=0.7
%         ] (1818,28) -- (1818,95) node[right] at (2000, 50) {\small{Average appearance: 1818 times}};
        
%         \addplot[
%             lightc!80!black,
%             line width=1mm,
%             % opacity=0.7
%             % mark=x,
%         ] % lifestyle
%             coordinates{
%                 (100, 27.94)
%                 (200, 59.58)
%                 (300, 66.36)
%                 (400, 70.75)
%                 (500, 73.94)
%                 (600, 76.34)
%                 (700, 78.17)
%                 (800, 79.60)
%                 (900, 80.70)
%                 (1000, 81.74)
%                 (1100, 82.57)
%                 (1200, 83.30)
%                 (1300, 84.02)
%                 (1400, 84.64)
%                 (1500, 85.19)
%                 (1600, 85.65)
%                 (1700, 86.08)
%                 (1800, 86.52)
%                 (1900, 86.89)
%                 (2000, 87.25)
%                 (2100, 87.61)
%                 (2200, 87.95)
%                 (2300, 88.24)
%                 (2400, 88.50)
%                 (2500, 88.78)
%                 (2600, 89.02)
%                 (2700, 89.30)
%                 (2800, 89.51)
%                 (2900, 89.75)
%                 (3000, 89.97)
%                 (3100, 90.20)
%                 (3200, 90.40)
%                 (3300, 90.61)
%                 (3400, 90.79)
%                 (3500, 90.95)
%                 (3600, 91.12)
%                 (3700, 91.29)
%                 (3800, 91.43)
%                 (3900, 91.58)
%                 (4000, 91.72)
%                 (4100, 91.87)
%                 (4200, 92.02)
%                 (4300, 92.17)
%                 (4400, 92.30)
%                 (4500, 92.42)
%                 (4600, 92.55)
%                 (4700, 92.67)
%                 (4800, 92.79)
%                 (4900, 92.90)
%                 (5000, 93.01)
%                 (5100, 93.12)
%                 (5200, 93.23)
%                 (5300, 93.30)
%                 (5400, 93.38)
%                 (5500, 93.49)
%                 (5600, 93.58)
%                 (5700, 93.66)
%                 (5800, 93.74)
%                 (5900, 93.80)
%                 (6000, 93.87)
%                 (6100, 93.94)
%                 (6200, 94.03)
%                 (6300, 94.10)
%                 (6400, 94.19)
%                 (6500, 94.27)
%                 (6600, 94.37)
%                 (6700, 94.44)
%                 (6800, 94.51)
%                 (6900, 94.59)
%                 (7000, 94.67)
%                 (7100, 94.73)
%                 (7200, 94.80)
%                 (7300, 94.85)
%                 (7400, 94.91)
%                 (7500, 94.97)
%             };
%     \end{axis}
% \end{tikzpicture}


% % \end{tabular}
% % }
% % \caption{\label{fig:appearance} The relation between news appearance times and proportion of news articles. Each point (x, y) represents y \% of news articles appear less than x times within a training epoch.
% % }
% % \end{figure}


==> tables/big-table-backup.tex <==
\newcommand{\coesmall}{\textcolor[HTML]{3E7A3E}}  % acceptable color
\newcommand{\coemedian}{\textcolor[HTML]{DB3636}}  % unacceptable color
\newcommand{\coelarge}{\textcolor[HTML]{DB3636}}  % unacceptable color


\begin{table*}[t]

\centering
\renewcommand\arraystretch{1.2}
% \setlength\tabcolsep{4pt}

\resizebox{0.95\linewidth}{!}{
\begin{tabular}{llcccccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Dataset}}  & \multicolumn{6}{c}{\textbf{MIND-small}} & \multicolumn{6}{c}{\textbf{MIND-large}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
&  & \multicolumn{4}{c}{\textbf{Matching}} & \multicolumn{2}{c}{\textbf{Ranking}} & \multicolumn{4}{c}{\textbf{Matching}} & \multicolumn{2}{c}{\textbf{Ranking}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12} \cmidrule(lr){13-14}
\multicolumn{2}{c}{\textbf{Method}} & \textbf{NAML} & \textbf{LSTUR} & \textbf{NRMS} & \textbf{BST} & \textbf{DCN} & \textbf{DIN} & \textbf{NAML} & \textbf{LSTUR} & \textbf{NRMS} & \textbf{BST} & \textbf{DCN} & \textbf{DIN} \\
\midrule
\multirow{5}{*}{\ete ID-based}
 & AUC & 50.13 & 51.04 & 54.84 & 50.09 & 53.92 & 55.95 
       & 52.98 & 54.98 & 57.59 & 52.10 & 57.41 & 57.36 \\
 & MRR & 23.01 & 22.90 & 26.53 & 22.13 & 25.18 & 25.88
       & 24.52 & 25.99 & 27.41 & 24.81 & 26.76 & 26.70 \\
 & N@5 & 22.35 & 22.31 & 26.34 & 21.59 & 24.43 & 25.95
       & 24.12 & 25.64 & 27.05 & 24.63 & 26.90 & 26.84 \\
 & \ce & 19    & 20    & 28    & 38    & 50    & 58 
       & 294   & 353   & 471   & 555   & 791   & 926   \\
 & ApC & 0.68  & 5.20  & 17.29 & 0.24  & 7.84  & 10.26 
       & 1.01  & 1.41  & 1.61  & 0.38  & 0.94  & 0.79  \\
\midrule
\multirow{5}{*}{\ete Text-based} 
 & AUC & 60.14 & 61.27 & 62.21 & 60.51 & 62.63 & 62.90
       & 63.03 & 63.89 & 64.12 & 63.28 & 63.88 & 64.02 \\
 & MRR & 28.93 & 29.64 & 30.19 & 28.59 & 29.73 & 30.06
       & 30.40 & 31.24 & 31.77 & 30.73 & 31.65 & 31.98 \\
 & N@5 & 29.33 & 30.28 & 31.10 & 29.09 & 30.52 & 30.65
       & 31.82 & 32.15 & 32.64 & 31.95 & 32.40 & 33.00 \\
 & \ce & 42    & 58    & 62    & 53    & 75    & 79 
       & 648   & 892   & 1010  & 1212  & 1684  & 1746  \\
 & ApC & 24.14 & 19.43 & 19.69 & 19.83 & 16.84 & 16.33 
       & 2.01  & 1.56  & 1.40  & 1.09  & 0.82  & 0.80  \\
\midrule

% \midrule
\multirow{5}{*}{\ptft BERT-token}
 & AUC & 60.68 & 61.26 & 62.82 & 60.63 & 61.13 & 62.84
       & 63.62 & 64.11 & 64.02 & 64.08 & 64.53 & 64.31 \\
 & MRR & 29.42 & 29.87 & 30.78 & 30.52 & 28.19 & 30.12
       & 31.44 & 31.60 & 31.55 & 31.42 & 32.02 & 32.15 \\
 & N@5 & 29.83 & 30.47 & 31.30 & 31.04 & 28.63 & 30.85
       & 32.09 & 32.28 & 32.20 & 32.05 & 32.98 & 33.10 \\
 & \ce & 42    & 58    & 62    & 53    & 75    & 79 
       & 648   & 892   & 1010  & 1212  & 1684  & 1746  \\
 & ApC & 25.43 & 19.41 & 20.68 & 20.06 & 14.84 & 16.25 
       & 2.10  & 1.58  & 1.39  & 1.16  & 0.86  & 0.82  \\
\midrule
\multirow{5}{*}{\ptft PLMNR}
 & AUC & 62.06 & 63.64 & 62.53 & 64.40 & 63.32 & 63.26
       & 65.19 & 65.73 & 65.57 & 66.03 & 65.42 & 65.31 \\
 & MRR & 31.66 & 31.74 & 30.74 & 32.21 & 32.00 & 31.83
       & 32.74 & 33.18 & 32.94 & 33.40 & 32.85 & 32.68 \\
 & N@5 & 32.25 & 32.72 & 31.31 & 33.34 & 32.58 & 32.40
       & 33.77 & 34.26 & 34.13 & 34.70 & 33.99 & 33.70 \\
 & \ce & 178   & 202   & 252   & 505   & 277   & 606 
       & 2527  & 3032  & 4043  & 8086  & 6570  & 10108 \\
 & ApC & 6.78  & 6.75  & 4.97  & 2.85  & 4.81  & 2.51 
       & 0.60  & 0.52  & 0.39  & 0.20  & 0.23  & 0.15  \\
\midrule
\multirow{5}{*}{\nrl BERT-news}
 & AUC & 60.62 & 61.09 & 60.94 & 60.81 & 62.65 & 62.40
       & 63.02 & 63.62 & 63.40 & 62.94 & 64.29 & 63.75 \\
 & MRR & 29.31 & 29.26 & 29.31 & 29.04 & 30.92 & 30.75
       & 31.23 & 31.59 & 31.38 & 30.56 & 32.60 & 31.58 \\
 & N@5 & 29.71 & 29.60 & 29.65 & 29.38 & 31.37 & 32.44
       & 31.79 & 32.30 & 32.16 & 31.83 & 33.63 & 32.43 \\
 & \ce & 22    & 23    & 33    & 38    & 67    & 58 
       & 353   & 404   & 505   & 640   & 1010  & 1010  \\
 & ApC & 48.27 & 48.22 & 33.15 & 28.45 & 18.88 & 21.37 
       & 3.69  & 3.37  & 2.65  & 2.02  & 1.41  & 1.36  \\
\midrule
\multirow{5}{*}{\nrl MFT-news}
 & AUC & 62.95 & 62.16 & 62.95 & 62.43 & 64.57 & 63.12
       & 64.78 & 64.88 & 64.34 & 65.33 & 65.44 & 64.53 \\
 & MRR & 31.26 & 31.00 & 31.18 & 30.42 & 32.60 & 31.28
       & 32.64 & 32.94 & 32.93 & 33.29 & 33.04 & 32.72 \\
 & N@5 & 32.01 & 31.79 & 32.10 & 30.94 & 33.48 & 32.01
       & 33.66 & 34.00 & 33.95 & 34.35 & 34.03 & 33.58 \\
 & \ce & 22    & 23    & 33    & 38    & 67    & 58 
       & 353   & 404   & 505   & 640   & 1010  & 1010 \\
 & ApC & \textbf{58.86} & \textbf{52.87} & \textbf{39.24} & \textbf{32.71} & \textbf{21.75} & \textbf{22.62} 
       & \textbf{4.19}  & \textbf{3.68}  & \textbf{2.84}  & \textbf{2.40}  & \textbf{1.53}  & \textbf{1.44} \\
\bottomrule
\end{tabular}
}

\caption{Comparison of different variants of different recommendation baselines. Blue circle ( \ete) indicates using the end-to-end framework. Orange circle ( \ptft) indicates using the pretrain-finetune framework. Green circle ( \nrl) indicates using the proposed GNR framework.}
\label{tab:big-table}

\end{table*}

